Analysis of Adversarial Image Manipulations

As virtual and physical identity grow increasingly intertwined, the importance of privacy and security in the online sphere becomes paramount. In recent years, multiple news stories have emerged of private companies scraping web content and doing research with or selling the data. Images uploaded online can be scraped without users' consent or knowledge. Users of social media platforms whose images are scraped may be at risk of being identified in other uploaded images or in real-world identification situations. This paper investigates how simple, accessible image manipulation techniques affect the accuracy of facial recognition software in identifying an individual's various face images based on one unique image.

==> Figures/filterSnippet.tex <==
\begin{lstlisting}[language=Python, caption=Coloration Filters Code]
from PIL import Image
import pilgram as p
import os

dir = `500ProbeImages'

for image in os.listdir(dir):
    path = os.path.join(dir, image)
    im = Image.open(path)
    s = im.split('_')[0]
    
    p.lofi(im).save(s + '_lofi.jpg')
    p.earlybird(im).save(s + '_eb.jpg')
    p.moon(im).save(s + '_moon.jpg') 
    p.X-Pro II(im).save(s + '_X-Pro II.jpg')
\end{lstlisting}
